Non-Parametric Manifold Learning

We introduce an estimator for distances in a compact Riemannian manifold based on graph Laplacian estimates of the Laplace-Beltrami operator. We upper bound the error in the estimate of manifold distances, or more precisely an estimate of a spectrally truncated variant of manifold distance of interest in non-commutative geometry (cf. [Connes and Suijelekom, 2020]), in terms of spectral errors in the graph Laplacian estimates and, implicitly, several geometric properties of the manifold. A consequence is a proof of consistency for (untruncated) manifold distances. The estimator resembles, and in fact its convergence properties are derived from, a special case of the Kontorovic dual reformulation of Wasserstein distance known as Connes' Distance Formula.

==> rates.tex <==
\newcommand{\GradientProductError}[2]{{#1}^{3}#2^2\nu(#1,N)}
\newcommand{\LinearError}[2]{#1\err_{\operator;#1}#2}
\newcommand{\ProductError}{q^2\|f\|_\infty^2|\lambda_{q}|^{\nicefrac{(d-1)}{2}}\nu(r,N)}
\newcommand{\QuadraticError}{r^{4}\|f\|_\infty^2(\nu(r,N)+\err_{\operator;r})}
\newcommand{\DoubleGradientError}{k^2\|f\|_\infty(1+k\|f\|_\infty\nu(k,N))}
\newcommand{\ApproximationError}{r^{4}\|f\|_\infty^2(\nu(r,N)+\err_{\operator;r}+\delta)}
\newcommand{\MISE}{\ApproximationError{}}
\newcommand{\IntroMISE}{r^{4}\|f\|_\infty^2(\sum_{\ell=r}^\infty\ell^{-N}+\err_{\hat{\graphlaplacian};r}+\delta)}
\newcommand{\IntroStochasticMISE}{r^{4}\|f\|_\infty^2(\sum_{\ell=r}^\infty\ell^{-N}+\err_{\hat{\graphlaplacian}_n;r}+\delta_n)}


